Parameterized Complexity Classification for Interval Constraints

Constraint satisfaction problems form a nicely behaved class of problems that lends itself to complexity classification results. From the point of view of parameterized complexity, a natural task is to classify the parameterized complexity of MinCSP problems parameterized by the number of unsatisfied constraints. In other words, we ask whether we can delete at most $k$ constraints, where $k$ is the parameter, to get a satisfiable instance. In this work, we take a step towards classifying the parameterized complexity for an important infinite-domain CSP: Allen's interval algebra (IA). This CSP has closed intervals with rational endpoints as domain values and employs a set $A$ of 13 basic comparison relations such as ``precedes'' or ``during'' for relating intervals. IA is a highly influential and well-studied formalism within AI and qualitative reasoning that has numerous applications in, for instance, planning, natural language processing and molecular biology. We provide an FPT vs. W[1]-hard dichotomy for MinCSP$(\Gamma)$ for all $\Gamma \subseteq A$. IA is sometimes extended with unions of the relations in $A$ or first-order definable relations over $A$, but extending our results to these cases would require first solving the parameterized complexity of Directed Symmetric Multicut, which is a notorious open problem. Already in this limited setting, we uncover connections to new variants of graph cut and separation problems. This includes hardness proofs for simultaneous cuts or feedback arc set problems in directed graphs, as well as new tractable cases with algorithms based on the recently introduced flow augmentation technique. Given the intractability of MinCSP$(A)$ in general, we then consider (parameterized) approximation algorithms and present a factor-$2$ fpt-approximation algorithm.

==> figures/rcc5-figure.tex <==
\def\rccfigwidth{0.1\textwidth}
\begin{figure}[tb]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.75]
            \draw (0,0) circle (1);
            \draw[dashed] (0,0) circle (1);
            \draw (-0.33,0) node {$X$};
            \draw (0.33,0) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf EQ}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.5]
            \draw (0,0.75) circle (1);
            \draw[dashed] (0,-0.75) circle (1);
            \draw (0,0.75) node {$X$};
            \draw (0,-0.75) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf PO}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}
            \draw (-0.3,0) circle (0.5);
            \draw (-0.3,0) node {$X$};
            \draw[dashed] (0,0) circle (1);
            \draw (0.5,0) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf PP}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}
            \draw[dashed] (-0.3,0) circle (0.5);
            \draw (-0.3,0) node {$Y$};
            \draw (0,0) circle (1);
            \draw (0.5,0) node {$X$};
        \end{tikzpicture}
        \caption{${\sf PP}^{-1}(X,Y)$}
    \end{subfigure}

    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.5]
            \draw (0,1.1) circle (1);
            \draw (0,1.1) node {$X$};
            \draw[dashed] (0,-1.1) circle (1);
            \draw (0,-1.1) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf DR}(X,Y)$}
    \end{subfigure}
    
    \caption{Illustration of the relations of RCC5 with 
    two-dimensional disks.}
    \label{fig:rcc5}
\end{figure}

==> figures/rcc8-figure.tex <==
\def\rccfigwidth{0.1\textwidth}
\begin{figure}[tb]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.75]
            \draw (0,0) circle (1);
            \draw[dashed] (0,0) circle (1);
            \draw (-0.33,0) node {$X$};
            \draw (0.33,0) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf EQ}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.5]
            \draw (0,0.75) circle (1);
            \draw[dashed] (0,-0.75) circle (1);
            \draw (0,0.75) node {$X$};
            \draw (0,-0.75) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf PO}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}
            \draw (-0.3,0) circle (0.5);
            \draw (-0.3,0) node {$X$};
            \draw[dashed] (0,0) circle (1);
            \draw (0.5,0) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf NTPP}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}
            \draw[dashed] (-0.3,0) circle (0.5);
            \draw (-0.3,0) node {$Y$};
            \draw (0,0) circle (1);
            \draw (0.5,0) node {$X$};
        \end{tikzpicture}
        \caption{${\sf NTPP}^{-1}(X,Y)$}
    \end{subfigure}

    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.5]
            \draw (0,1) circle (1);
            \draw (0,1) node {$X$};
            \draw[dashed] (0,-1) circle (1);
            \draw (0,-1) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf EC}(X,Y)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\rccfigwidth}
        \centering
        \begin{tikzpicture}[scale=0.5]
            \draw (0,1.1) circle (1);
            \draw (0,1.1) node {$X$};
            \draw[dashed] (0,-1.1) circle (1);
            \draw (0,-1.1) node {$Y$};
        \end{tikzpicture}
        \caption{${\sf DC}(X,Y)$}
    \end{subfigure}
    
    \caption{Illustration of the relations of RCC5 with 
    two-dimensional disks.}
    \label{fig:rcc8}
\end{figure}
